SoK: Towards Effective Automated Vulnerability Repair

The increasing prevalence of software vulnerabilities necessitates automated vulnerability repair (AVR) techniques. This Systematization of Knowledge (SoK) provides a comprehensive overview of the AVR landscape, encompassing both synthetic and real-world vulnerabilities. Through a systematic literature review and quantitative benchmarking across diverse datasets, methods, and strategies, we establish a taxonomy of existing AVR methodologies, categorizing them into template-guided, search-based, constraint-based, and learning-driven approaches. We evaluate the strengths and limitations of these approaches, highlighting common challenges and practical implications. Our comprehensive analysis of existing AVR methods reveals a diverse landscape with no single ``best'' approach. Learning-based methods excel in specific scenarios but lack complete program understanding, and both learning and non-learning methods face challenges with complex vulnerabilities. Additionally, we identify emerging trends and propose future research directions to advance the field of AVR. This SoK serves as a valuable resource for researchers and practitioners, offering a structured understanding of the current state-of-the-art and guiding future research and development in this critical domain.

==> commons/pkg.tex <==
% \usepackage[utf8]{inputenc}

% it, be sure to load this package with the cmex10 option to ensure that
% only type 1 fonts will utilized at all point sizes. Without this option,
% it is possible that some math symbols, particularly those within
% footnotes, will be rendered in bitmap form which will result in a
% document that can not be IEEE Xplore compliant!
% \usepackage{amsmath}
% \usepackage{graphicx}
% % it is a good idea to load it with the tight package option to reduce
% % the amount of white space around the subfigures. 
% \usepackage[tight,footnotesize]{subfigure}
% %\usepackage[caption=false,font=footnotesize]{subfig}
% \usepackage{multirow}
% \usepackage{fancyvrb}
% \usepackage[flushleft, online]{threeparttable}
% % Loading the cite package will
% % result in citation numbers being automatically sorted and properly
% % "compressed/ranged". e.g., [1], [9], [2], [7], [5], [6] without using
% % cite.sty will become [1], [2], [5]--[7], [9] using cite.sty. cite.sty's
% % \cite will automatically add leading space,
% \usepackage{cite}
% \usepackage{xurl}
% \usepackage{array}
% \usepackage{algorithmic}
% \usepackage{booktabs}
% \usepackage{xcolor}
% \usepackage{emoji}
% \usepackage{twemoji}
% \usepackage{fontspec}

% \usepackage{fontspec}
